Interstellar Detection of the Highly Polar Five-Membered Ring Cyanocyclopentadiene

Much like six-membered rings, five-membered rings are ubiquitous in organic chemistry, frequently serving as the building blocks for larger molecules, including many of biochemical importance. From a combination of laboratory rotational spectroscopy and a sensitive spectral line survey in the radio band toward the starless cloud core TMC-1, we report the astronomical detection of 1-cyano-1,3-cyclopentadiene, $c$-C$_5$H$_5$CN}, a highly polar, cyano derivative of cyclopentadiene, $c$-C$_5$H$_6$. The derived abundance of $c$-C$_5$H$_5$CN} is far greater than predicted from astrochemical models which well reproduce the abundance of many carbon chains. This finding implies either an important production mechanism or a large reservoir of aromatic material may need to be considered. The apparent absence of its closely-related isomer, 2-cyano-1,3-cyclopentadiene, may arise from its lower stability or be indicative of a more selective pathway for formation of the 1-cyano isomer, perhaps one starting from acyclic precursors. The absence of N-heterocycles such as pyrrole and pyridine is discussed in light of the astronomical finding.

==> 1-cyano-CPD_stack_table.tex <==
\begin{table*}
\centering
\caption{\ce{1-CYANO-CPD} best-fit parameters from MCMC analysis}
\begin{tabular}{c c c c c c}
\toprule
\multirow{2}{*}{Component}&	$v_{lsr}$					&	Size					&	\multicolumn{1}{c}{$N_T^\dagger$}					&	$T_{ex}$							&	$\Delta V$		\\
			&	(km s$^{-1}$)				&	($^{\prime\prime}$)		&	\multicolumn{1}{c}{(10$^{11}$ cm$^{-2}$)}		&	(K)								&	(km s$^{-1}$)	\\
\midrule
\hspace{0.1em}\vspace{-0.5em}\\
C1	&	$5.599^{+0.010}_{-0.008}$	&	$99^{+2}_{-1}$	&	$3.73^{+0.91}_{-0.82}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.123^{+0.011}_{-0.011}$\\
\hspace{0.1em}\vspace{-0.5em}\\
C2	&	$5.764^{+0.004}_{-0.003}$	&	$65^{+4}_{-3}$	&	$2.44^{+1.04}_{-1.04}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.123^{+0.011}_{-0.011}$\\
\hspace{0.1em}\vspace{-0.5em}\\
C3	&	$5.882^{+0.008}_{-0.008}$	&	$266^{+2}_{-2}$	&	$4.75^{+1.08}_{-0.90}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.123^{+0.011}_{-0.011}$\\
\hspace{0.1em}\vspace{-0.5em}\\
C4	&	$6.016^{+0.004}_{-0.003}$	&	$262^{+2}_{-2}$	&	$2.39^{+0.85}_{-0.75}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.123^{+0.011}_{-0.011}$\\
\hspace{0.1em}\vspace{-0.5em}\\
\midrule
$N_T$ (Total)$^{\dagger\dagger}$	&	 \multicolumn{5}{c}{$1.3^{+0.39}_{-0.35}\times 10^{12}$~cm$^{-2}$}\\
\bottomrule
\end{tabular}

\begin{minipage}{0.75\textwidth}
	\footnotesize
	\textbf{Note} -- The quoted uncertainties represent the 16$^{th}$ and 84$^{th}$ percentile ($1\sigma$ for a Gaussian distribution) uncertainties.\\
	$^\dagger$Column density values are highly covariant with the derived source sizes.  The marginalized uncertainties on the column densities are therefore dominated by the largely unconstrained nature of the source sizes, and not by the signal-to-noise of the observations.  See Fig.~\ref{1-cyano-CPD_triangle} for a covariance plot, and \citealt{HC11N} for a detailed explanation of the methods used to constrain these quantities and derive the uncertainties.\\
	$^{\dagger\dagger}$Uncertainties derived by adding the uncertainties of the individual components in quadrature.
\end{minipage}

\label{1-cyano-CPD_results}

\end{table*}


==> 2-cyano-CPD_stack_table.tex <==
\begin{table*}
\centering
\caption{\ce{2-CYANO-CPD} best-fit parameters from MCMC analysis}
\begin{tabular}{c c c c c c}
\toprule
\multirow{2}{*}{Component}&	$v_{lsr}$					&	Size					&	\multicolumn{1}{c}{$N_T^\dagger$}					&	$T_{ex}$							&	$\Delta V$		\\
			&	(km s$^{-1}$)				&	($^{\prime\prime}$)		&	\multicolumn{1}{c}{(10$^{11}$ cm$^{-2}$)}		&	(K)								&	(km s$^{-1}$)	\\
\midrule
\hspace{0.1em}\vspace{-0.5em}\\
C1	&	$5.595^{+0.007}_{-0.008}$	&	$99^{+1}_{-1}$	&	$1.41^{+0.66}_{-0.56}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.122^{+0.011}_{-0.009}$\\
\hspace{0.1em}\vspace{-0.5em}\\
C2	&	$5.764^{+0.004}_{-0.005}$	&	$65^{+1}_{-1}$	&	$1.51^{+0.70}_{-0.68}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.122^{+0.011}_{-0.009}$\\
\hspace{0.1em}\vspace{-0.5em}\\
C3	&	$5.886^{+0.009}_{-0.009}$	&	$265^{+0}_{-1}$	&	$0.78^{+0.95}_{-0.54}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.122^{+0.011}_{-0.009}$\\
\hspace{0.1em}\vspace{-0.5em}\\
C4	&	$6.016^{+0.003}_{-0.004}$	&	$262^{+1}_{-0}$	&	$0.75^{+0.57}_{-0.45}$	&	$6.1^{+0.0}_{-0.0}$	&	$0.122^{+0.011}_{-0.009}$\\
\hspace{0.1em}\vspace{-0.5em}\\
\midrule
$N_T$ (Total)$^{\dagger\dagger}$	&	 \multicolumn{5}{c}{$4.5^{+2.88}_{-2.23}\times 10^{11}$~cm$^{-2}$}\\
\bottomrule
\end{tabular}

\begin{minipage}{0.75\textwidth}
	\footnotesize
	\textbf{Note} -- The quoted uncertainties represent the 16$^{th}$ and 84$^{th}$ percentile ($1\sigma$ for a Gaussian distribution) uncertainties.\\
	$^\dagger$Column density values are highly covariant with the derived source sizes.  The marginalized uncertainties on the column densities are therefore dominated by the largely unconstrained nature of the source sizes, and not by the signal-to-noise of the observations.  See Fig.~\ref{2-cyano-CPD_triangle} for a covariance plot, and \citealt{HC11N} for a detailed explanation of the methods used to constrain these quantities and derive the uncertainties.\\
	$^{\dagger\dagger}$Uncertainties derived by adding the uncertainties of the individual components in quadrature.
\end{minipage}

\label{2-cyano-CPD_results}

\end{table*}

